Oscillations between Grid-Forming Converters in Weakly Connected Offshore WPPs

This paper studies control interactions between grid-forming (GFM) converters exhibited by power and frequency oscillations in a weakly connected offshore wind power plant (WPP). Two GFM controls are considered, namely virtual synchronous machine (VSM) and virtual admittance (VAdm) based GFM. The GFM control methods are implemented in wind turbine generators (WTGs) of a verified aggregated model of a WPP and the control interaction between these GFM WTGs is studied for several cases: cases with the same GFM control methods, and cases with different GFM control methods. A sensitivity analysis is performed for the observed oscillations to understand which system parameter affects the oscillations the most. Several solution methods are proposed and the inapplicability of some of the conventional solution methods are elaborated in this paper.

==> bib/Bibliography.tex <==
@ARTICLE{8742900,
  author={Li, Yin and Fan, Lingling and Miao, Zhixin},
  journal={IEEE Transactions on Power Systems}, 
  title={Wind in Weak Grids: Low-Frequency Oscillations, Subsynchronous Oscillations, and Torsional Interactions}, 
  year={2020},
  volume={35},
  number={1},
  pages={109-118},
  doi={10.1109/TPWRS.2019.2924412}}

@ARTICLE{7944679,
  author={Fan, Lingling and Miao, Zhixin},
  journal={IEEE Transactions on Sustainable Energy}, 
  title={An Explanation of Oscillations Due to Wind Power Plants Weak Grid Interconnection}, 
  year={2018},
  volume={9},
  number={1},
  pages={488-490},
  doi={10.1109/TSTE.2017.2713980}}

@article{ghimire2023gridforming,
  title={Grid-Forming Control Methods for Weakly Connected Offshore WPPs},
  author={Ghimire, Sulav and Kkuni, Kanakesh V and Jakobsen, Simon C and Knueppel, Thyge and Jensen, Kim H and Guest, Emerson and Rasmussen, Tonny W and Yang, Guangya},
  journal={22nd Wind and Solar Integration Workshop},
  year={2023}
}

@INPROCEEDINGS{6344713,
  author={Huang, Shun-Hsien and Schmall, John and Conto, Jose and Adams, John and Zhang, Yang and Carter, Cathey},
  booktitle={2012 IEEE Power and Energy Society General Meeting}, 
  title={Voltage control challenges on weak grids with high penetration of wind generation: ERCOT experience}, 
  year={2012},
  volume={},
  number={},
  pages={1-7},
  doi={10.1109/PESGM.2012.6344713}}

@ARTICLE{7878693,
  author={Liu, Huakun and Xie, Xiaorong and He, Jingbo and Xu, Tao and Yu, Zhao and Wang, Chao and Zhang, Chuanyu},
  journal={IEEE Transactions on Power Systems}, 
  title={Subsynchronous Interaction Between Direct-Drive PMSG Based Wind Farms and Weak AC Networks}, 
  year={2017},
  volume={32},
  number={6},
  pages={4708-4720},
  doi={10.1109/TPWRS.2017.2682197}}

@techreport{connectionwindfarms,
  type = {Technical Brochures},
  title = {Connection of Wind Farms to Weak AC Networks},
  author = {{Working Group on Wind Farm Connection}},
  year = {2016},
  institution = {CIGRE Study Committee WG B4.62},
  url = {https://e-cigre.org/publication/671-connection-of-wind-farms-to-weak-ac-networks},
}

@article{kundur2017power,
  title={Power system dynamics and stability},
  author={Kundur, Prabha S and Balu, Neal J and Lauby, Mark G},
  journal={Power system stability and control},
  volume={3},
  pages={700--701},
  year={2017},
  publisher={McGraw-Hill}
}

@INPROCEEDINGS{9494824,
  author={Avazov, Artur and Colas, Frédéric and Beerten, Jef and Guillaud, Xavier},
  booktitle={2021 IEEE Madrid PowerTech}, 
  title={Damping of Torsional Vibrations in a Type-IV Wind Turbine Interfaced to a Grid-Forming Converter}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/PowerTech46648.2021.9494824}}

@article{ROKROK2020106765,
title = {Classification and dynamic assessment of droop-based grid-forming control schemes: Application in HVDC systems},
journal = {Electric Power Systems Research},
volume = {189},
pages = {106765},
year = {2020},
issn = {0378-7796},
doi = {https://doi.org/10.1016/j.epsr.2020.106765},
url = {https://www.sciencedirect.com/science/article/pii/S037877962030568X},
author = {Ebrahim Rokrok and Taoufik Qoria and Antoine Bruyere and Bruno Francois and Xavier Guillaud},
keywords = {Droop control, Grid-forming control, HVDC systems, Inertia support, Power regulation}
}

@ARTICLE{6361459,
  author={Licari, John and Ugalde-Loo, Carlos E. and Ekanayake, Janaka B. and Jenkins, Nicholas},
  journal={IEEE Transactions on Energy Conversion}, 
  title={Damping of Torsional Vibrations in a Variable-Speed Wind Turbine}, 
  year={2013},
  volume={28},
  number={1},
  pages={172-180},
  doi={10.1109/TEC.2012.2224868}}

@ARTICLE{9625987,
  author={Rodríguez-Amenedo, José Luis and Gómez, Santiago Arnaltes},
  journal={IEEE Access}, 
  title={Damping Low-Frequency Oscillations in Power Systems Using Grid-Forming Converters}, 
  year={2021},
  volume={9},
  number={},
  pages={158984-158997},
  doi={10.1109/ACCESS.2021.3130333}}

